MARCO: Multi-Agent Real-time Chat Orchestration

Large language model advancements have enabled the development of multi-agent frameworks to tackle complex, real-world problems such as to automate tasks that require interactions with diverse tools, reasoning, and human collaboration. We present MARCO, a Multi-Agent Real-time Chat Orchestration framework for automating tasks using LLMs. MARCO addresses key challenges in utilizing LLMs for complex, multi-step task execution. It incorporates robust guardrails to steer LLM behavior, validate outputs, and recover from errors that stem from inconsistent output formatting, function and parameter hallucination, and lack of domain knowledge. Through extensive experiments we demonstrate MARCO's superior performance with 94.48% and 92.74% accuracy on task execution for Digital Restaurant Service Platform conversations and Retail conversations datasets respectively along with 44.91% improved latency and 33.71% cost reduction. We also report effects of guardrails in performance gain along with comparisons of various LLM models, both open-source and proprietary. The modular and generic design of MARCO allows it to be adapted for automating tasks across domains and to execute complex usecases through multi-turn interactions.

==> content/03-approach/03-2-approach-marco_components/03-2-3-marco_components-rag.tex <==
\subsubsection{RAG} \label{subsub_sec:approach-rag}

\textcolor{red}{When a user query is classified as an \emph{I = Info} intent, the chat conversation history is redirected to Retrieval Augmented Generation module (RAG), which first rephrases the multi-turn conversation along with latest user query into a short question using \emph{claude-instant-v1} and then finds the top-5 relevant context chunks from index store saved in AWS OpenSearch, followed by answer generation with the context and rephrased query using \emph{claude-instant-v1}. The implementation details of RAG module are out of scope for this paper.}
%as it has been extensively explored in \textcolor{red}{previous works~\cite{}}.


==> content/figures/lfo_workflow.tex <==
% \begin{figure}[htbp]
%   \centering
%   \includegraphics[width=0.9\columnwidth]{content/images/lfo_workflow.png}
%   \caption{An example retail usecase workflow diagram of Lost Featured Offer usecase, to show the complexity of retail workflow automation.}
%   \label{fig:lfo_workflow}
% \end{figure}

\begin{figure*}[htbp]
  \centering
  \includegraphics[width=0.9\textwidth]{content/images/food_data_workflow.png}
  \caption{An example DRSP usecase task diagram of Net Promotion Score (NPS) usecase, to show the complexity of task automation.}
  \label{fig:food_app_nps_workflow}
\end{figure*}
